Finding The Greedy, Prodigal, and Suicidal Contracts at Scale

Smart contracts---stateful executable objects hosted on blockchains like Ethereum---carry billions of dollars worth of coins and cannot be updated once deployed. We present a new systematic characterization of a class of trace vulnerabilities, which result from analyzing multiple invocations of a contract over its lifetime. We focus attention on three example properties of such trace vulnerabilities: finding contracts that either lock funds indefinitely, leak them carelessly to arbitrary users, or can be killed by anyone. We implemented MAIAN, the first tool for precisely specifying and reasoning about trace properties, which employs inter-procedural symbolic analysis and concrete validator for exhibiting real exploits. Our analysis of nearly one million contracts flags 34,200 (2,365 distinct) contracts vulnerable, in 10 seconds per contract. On a subset of3,759 contracts which we sampled for concrete validation and manual analysis, we reproduce real exploits at a true positive rate of 89%, yielding exploits for3,686 contracts. Our tool finds exploits for the infamous Parity bug that indirectly locked 200 million dollars worth in Ether, which previous analyses failed to capture.

==> concreteval.tex <==
\label{sec:concval}

The concrete validation framework of \codename takes as input context the values of
transaction inputs found by the symbolic analysis engine.
%It exploits a contract 
The framework provides an execution environment equivalent to
the original execution  environment of  Ethereum framework. 
That is, on a private fork of Ethereum blockchain it checks
whether the properties mentioned in Section~\ref{sec:properties} hold for
corresponding bug category. It outputs whether
a candidate is true or false positive with respect to a bug
category flagged by the symbolic execution engine. 
%based on the results obtained from evaluating correctness of corresponding properties.

%\paragraph{Validation framework} 
To implement the validating framework, 
we add a new functionality to the official
go-ethereum package\cite{goEthereum} which allows us to fork the Ethereum
main chain at a block height of our choice. 
%
Once we fork the main chain, we mine on that fork without connecting to any peers on the Ethereum network, 
%, bythis, we are able to mine our own blocks without letting  the network know about them.  Consequently, 
and thus we are able to mine our own transactions  without
commiting them to the main chain. 
%One has to observe that 
%Note, we generate our own
%Ether, required for validating purposes. For instance, any transaction
%submitted to the blockchain requires gas  to be mined(executed) and in order
%to provide that gas, the sender's account needs to have Ether  balance. 
% During exploitation of a contract, 
%On our private chain, the initial contract state is its state at the block
%height where we have forked the main chain. 
%The contract's state may change with every
%invocation of the exploit. However,  once the validation process terminates,
%it leaves the contract's  state unchanged on the main chain since the mined
%blocks on our fork are never shown to the network.


\paragraph{Prodigal Contracts} The validation framework checks if a contract
leaks  Ether by sending to it the transactions with inputs provided by
the symbolic analysis engine. 
The transactions are sent by one of our accounts created previously. 
%(message sender) which does
%not mine, submits transactions to the network and our miner account mines
%these transactions . 
Once the transactions are executed, to test if the contract is a true positive the validation framework
checks whether the contract has sent Ether to our account. 
%the message sender to confirm whether  the candidate is a True Positive.  
If a verifying contract does not have Ether, our
framework first sends Ether to the contract and only then runs the exploit. 
%If the contract does not exist on main chain then the main chain can be forked at a
%block height where the contract exists, before exploiting it.


\paragraph{Suicidal Contracts} %In this case, 
In a similar fashion, the framework checks if a
contract can be killed after executing the transactions provided by the symbolic analysis engine 
on the forked chain. 
%performing the exploit on forked chain by a similar procedure described in the case of Prodigal contracts. 
Note, once a contract is killed, %its  storage fields are cleared on the blockchain and 
its bytecode is reset to \emph{'0x'}. % and  all its balance is sent to a specific address which is decided by the contracts logic. 
Our framework uses precisely this test to confirm the correctness of the exploit. 
%checks if  for the bytecode field after performing an exploit. 
%If a contract doesn't exist on the blockchain at that block height then fork can be started at a
%block height where  the contract exists.

\paragraph{Greedy Contracts} A strategy similar to the above two cannot be used to validate the exploits on contracts that lock Ether. However, during the bug finding process, our symbolic execution engine
checks firsthand whether a contract accepts Ether. % before checking for other properties.
Therefore, the validation framework can check if a contract is true positive by confirming that it accepts Ether and does not have \texttt{CALL}, \texttt{CALLCODE}, \texttt{DELEGATECALL}
or \texttt{SUICIDE} opcodes in its bytecode. In Section~\ref{sec:eval} we give examples of such contracts.


==> discussion.tex <==

\section{Discussion}
\label{sec:discussion}

\is{Discuss, how the properties can be strengthened.}


==> resultTable_copy.tex <==
\begin{table*}[t]
\centering
% \begin{tabular}{|p{1.2 cm}||p{1.2 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{0.8 cm}|p{1 cm}|p{1.5 cm}|p{0.7 cm}|p{1.2 cm}|}
\begin{tabular}{|p{2 cm}||p{1.8 cm}|p{1.5 cm}|p{1.5 cm}|p{1.5 cm}|p{1.8 cm}|p{2 cm}|p{2 cm}|}
\hline
Category & Flagged Candidates& With sources & W/o sources& Not Validated & Concretely Validated & TP (\textit{\% of TP}) & FP (\textit{\% of FP}) \\
\hline
Prodigal & 1504 & 16 & 1487 & 251 & 1253 & 1219 (\textit{97.28}) & 34 (\textit{2.71}) \\
\hline
Suicidal & 1495 & 7 & 1487 & 72 & 1423 & 1410 (\textit{99.09}) & 13 (\textit{0.91}) \\
\hline
Greedy & 61,362 & 177 & 61,185 & N/A & 25 & 11 (\textit{44}) & 14 (\textit{66})\\
\hline
Posthumous & 847 & - & 847 & 0 & 847 & 847 (\textit{100}) & 0 (\textit{0}) \\
\hline

\end{tabular}
\caption{Results using invocation depth $2$ at block height \texttt{BH}. Candidates created after the block height \texttt{BH} are not validated. In case of leak, contracts that do not have ether balance and that do not accept ether are not validated too. }
\label{fig:table}
\end{table*}
